Payment-failure times for random Lightning paths

We study a random process over graphs inspired by the way payments are executed in the Lightning Network, the main layer-two solution on top of Bitcoin. We first prove almost tight upper and lower bounds on the time it takes for a payment failure to occur, as a function of the number of nodes and the edge capacities, when the underlying graph is complete. Then, we show how such a random process is related to the edge-betweenness centrality measure and we prove upper and lower bounds for arbitrary graphs as a function of edge-betweenness and capacity. Finally, we validate our theoretical results by running extensive simulations over some classes of graphs, including snapshots of the real Lightning Network.

==> trunk/apx-furthersim.tex <==
\begin{center}
    \rule{5cm}{.5pt}
\end{center}

\section{Further simulations results and pictures}
In this part of the appendix we add some further simulation analysis.\\
Figures~\ref{fig:independent} and~\ref{fig:ring} illustrate the outcomes of multiple simulation runs for both the independent and even ring topologies. These simulations were conducted with a fixed number of nodes $n=4096$, while varying the channel capacity $c$ from $10$ to $3030$ in increments of $10$. This setup enables a comprehensive evaluation of the system's behavior, allowing us to compute the minimum, maximum, and average performance metrics across different capacity levels, and all the curves show an upward trend , demonstrating that the higher the capacity, the lower the probability of recording a failure.
The independent topology shows little variation around the average, indicating more stable performance. In contrast, the even ring topology has much larger variation, showing less consistent results. These differences are directly compared in Figure~\ref{fig:indp_cir}.
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{img/independent_graph_4096.png}
    \caption{ Simulated failure probabilities for independent chains
        systems with n = 4096 nodes and maximum capacity 3040.}
    \label{fig:independent}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{img/Ring_graph_4096.png}
    \caption{Simulated failure probabilities for ring chain
        systems with n = 4096 nodes and maximum capacity 3040.}
    \label{fig:ring}
\end{figure}

Figure~\ref{fig:multi-sim} histograms show how long transactions keep succeeding before the first failure. With the original distribution of capacity, most runs fail within about 8 transactions, especially when they are large. By contrast, the uniform distribution of capacity pushes failures far out, giving many more successful transactions across all sizes.

Finally, the optimized distribution of capacity for 100 k satoshis  further accentuates this effect: its distribution is shifted furthest to the right, demonstrating that the optimization procedure maximizes the minimum number of successful transactions before a failure compared to both the original and uniform distribution of capacity for the same transaction size.
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{img/Distribution_of_transaction.png}
    \caption{ Log-log histogram of simulations for sending multi-size transactions of 1k, 10k, and 100k satoshis.}
    \label{fig:multi-sim}
\end{figure}





==> trunk/preliminaries.tex <==
\section{Preliminaries on birth-and-death chains}\label{sec:preliminaries}
In this section we briefly recall some terminology and fundamental bounds about
\textit{birth-and-death} Markov chains.

A finite birth-and-death chain with absorbing boundary is a Markov chain
$\{X_t\,:\, t \in \mathbb{N}\}$ with state space
\[
\Omega = \{-k, -k+1, \dots, -1, 0, 1, \dots, k-1, k\}
\]
for some $k \in \mathbb{N}$, where 
\[
\Prob{}{X_{t+1} = -k \,|\, X_t = -k} = \Prob{}{X_{t+1} = k \,|\, X_t = k} = 1 \\
\]
and for each $j = -k+1, \dots, -1, 0, 1, \dots, k-1$,
\[
\begin{array}{rcl}
\Prob{}{X_{t+1} = j + 1\,|\, X_t = j} & = & p \\
\Prob{}{X_{t+1} = j - 1\,|\, X_t = j} & = & q \\
\Prob{}{X_{t+1} = j \,|\, X_t = j} & = & 1 - (p + q) \\
\end{array}
\]
for some non-negative $p$ and $q$ with $p + q < 1$. When $p = q = 1/2$ the
chain is said \textit{unbiased}.

\begin{center}
    \begin{small}
        \begin{tikzpicture}[scale=0.7]
            \node[circle,draw,color=blue,label=above:\textcolor{blue}{\small{$0$}}] (sj) at (0,0) {};
            \node[circle,draw,color=blue,label=above:\textcolor{blue}{\small{$1$}}] (sj+1) at (2,0) {};
            \node[circle,draw,color=blue,label=above:\textcolor{blue}{\small{$-1$}}] (sj-1) at (-2,0) {};
            \node[color=blue] (sdot) at (4,0) {$\dots\dots$};
            \node[circle,draw,color=blue,label=below:\textcolor{blue}{\small{$k$}}] (sn) at (6,0) {};
            \node[color=blue] (s-dot) at (-4,0) {$\dots\dots$};
            \node[circle,draw,color=blue,label=below:\textcolor{blue}{\small{$-k$}}] (s0) at (-6,0) {};
            \draw[->,>=stealth] (sj) edge [bend left] node[above] {$1/2$} (sj+1)
            (sj-1) edge [bend left] (sj);
            \draw[->,>=stealth] (sj+1) edge [bend left] (sdot)
            (sj+1) edge [bend left] (sj);
            \draw[->,>=stealth] (sj-1) edge [bend left](s-dot)
            (sj) edge [bend left] node[below] {$1/2$} (sj-1);
            \draw[->,>=stealth] (sn) edge [loop above] node[above] {$1$} (sn)
            (s-dot) edge [bend left] (s0)
            (s0) edge [loop above] node[above] {$1$} (s-dot)
            (sdot) edge [bend left] (sn);
        \end{tikzpicture}
    \end{small}
\end{center}

For unbiased birth-and-death chains it is well known that the expected time
before the chain hits the boundary starting from an arbitrary state $j$ is $k^2
- j^2$ (see, e.g., Chapter~2 in~\cite{levine2009markov}).
\begin{lemma}\label{apx:bdlemma}
    Let $\tau = \inf \{t \in \mathbb{N} \,:\, X_t = \pm k \}$ be the random variable
    indicating the first time in which the chain hits state $n$. The
    expectation of $\tau$ for the chain starting at an arbitrary state $j \in \Omega$ is
    \[
        \Expec{}{\tau \,|\, X_0 = j} = k^2 - j^2
    \]
\end{lemma}

To bound the probability that a finite chain hits the boundary before or after
a certain value, it is sometimes convenient to consider infinite
birth-and-death chains. The following Lemma~\ref{lemma:hittpos} is a well-known
bound (see, e.g., Exercise~2.10 in~\cite{levine2009markov}) for infinite chains
that can be used to give an upper bound on the probability that a chain hits
the boundary within a certain number of time steps, as shown in
Lemma~\ref{lemma:lbhitlemma}.

\begin{lemma}\label{lemma:hittpos}
    Let $\{X_t \,:\, t \in \mathbb{N} \}$ be an unbiased birth-and-death chain over
    $\mathbb{Z}$. For every time $t \in \mathbb{N}$ and for every \textit{target
        state} $k \in \mathbb{N}$ it holds that
    \[
        \Prob{0}{|X_t| \geqslant k}
        \leqslant \Prob{0}{\max_{i = 1, \dots, t} |X_i| \geqslant k}
        \leqslant 2 \Prob{0}{|X_t| \geqslant k}
    \]
\end{lemma}

The following lemma will be useful in the proofs of the lower bounds in
Theorems~\ref{thm:clique} and~\ref{thm:beetweenness}.

\begin{lemma}\label{lemma:lbhitlemma}
Let $\{X_t \,:\, t \in \mathbb{N} \}$ be an unbiased birth-and-death chain over
$\mathbb{Z}$, let $k \in \mathbb{N}$ be an integer and let $\tau$ be the random variable indicating the
first time the chain hits state $\pm k$,
\[
\tau = \inf\{t \in \mathbb{N} \,:\, |X_t| = k \}\,.
\]
Then, for every $t \in \mathbb{N}$ it holds that
\[
\Prob{0}{\tau \leqslant t} \leqslant 4 e^{-k^2 / (6t)}
\]
\end{lemma}
\begin{proof}
Observe that
\begin{align*}
\Prob{0}{\tau \leqslant t}
& = \Prob{0}{\max_{i = 1, \dots, t} |X_i| \geqslant k}
\leqslant 2 \Prob{0}{|X_t| \geqslant k}                 \\
& = 4 \Prob{0}{X_t \geqslant k}
\end{align*}
where in the second inequality we used Lemma~\ref{lemma:hittpos} and in the
third equality we used the symmetry of the process.

Now observe that
\[
\Prob{0}{X_t \geqslant k} = \Prob{}{B(t,1/2) \geqslant \frac{k+t}{2}}
\]
where with $B(t,1/2)$ we indicated a binomial random variable with parameters
$t$ and $1/2$. The thesis then follows from the Chernoff bound (see
Lemma~\ref{apx:chernoff} in the appendix).
\end{proof}




